Clustering extremal dependence structures via Wasserstein distances between angular measures

Grouping random vectors by their joint extremal behaviour is a recurring task in climate science, hydrology, and finance. Classical clustering is driven by typical observations, while existing extremal procedures either summarize dependence by a single coefficient or discretize the simplex in an ad hoc way. We propose a dissimilarity that compares complete angular measures by optimal transport: each angular measure is estimated above a high radial threshold, mapped from the simplex into a Euclidean space of Aitchison coordinates, and compared by the 1-Wasserstein distance. The methodology is fully nonparametric and requires no fitted model. The dissimilarities feed any distance-based clustering algorithm. Under intermediate-threshold asymptotics and mild moment and separation conditions, hierarchical clustering and partitioning around medoids based on them recovers the latent partition with probability tending to one. In simulations, the proposed approach matches established competitors when clusters differ mainly in the strength of extremal dependence and performs substantially better when equal-strength clusters differ in the shape of their angular measures, especially when asymmetry drives the separation. Applications to rain--snowmelt--runoff extremes in Swiss catchments and to extremal co-movement between international equity markets and the US market reveal hydrologically and economically interpretable groups.

==> unused_source_files/Clustering.tex <==
\subsection{Clustering compound event} \label{sec:Clustering}
In this section, we present state-of-the-art clustering methods for compound events. Let $n\geq 2$ and $p\geq2$, and consider $\mathcal{X}=\{\boldsymbol{X}_1,\dots,\boldsymbol{X}_n\}$, a set of $p$-dimensional continuous random vectors. Each random vector $\boldsymbol{X_i}=\left(X_i^{(1)},\dots,X_i^{(p)} \right)$ is associated with a random sample $(\boldsymbol{x_{it}})_{t=1,\dots,T}$. Think of $n$ as representing different sites where $p$ variables are recorded. The goal is to find a partition of $\mathcal{X}$ by using the dependence between its elements.
A common methodology can be described in three steps:
\begin{enumerate}
    \item Find a dissimilarity measure to compare random vectors in $\mathcal{X}$.
    \item Given the dissimilarity measure, construct an $(n \times n)$ "distance" matrix.
    \item Finally, use this matrix as input for a clustering algorithm such as k-medoid or hierarchical clustering. 
\end{enumerate}

\subsubsection{Dissimilarity measure based on the Kullback–Leibler (KL) divergence}
\citet{vignotto2021clustering} proposed a dissimilarity measure based on the Kullback–Leibler (KL) divergence, tailored to the framework of extreme value theory \citep{naveau2014non}. For two $p$-variate random vectors $\boldsymbol{X}_1$ and $\boldsymbol{X}_2$, they defined the divergence on the tails of the distributions after normalizing the marginal distributions to standard Pareto distributions. For a univariate random variable $X$ with distribution function $F$, this can be done empirically by $1/(1-\hat{F}(X))$. To define which areas are considered extreme, a risk function $r:\mathbb{R}^p \rightarrow \mathbb{R}$ is computed on the Pareto scale. Different choices for $r$ exist, such as the maximum function $r(\boldsymbol{x})=\max(x^{(1)},\dots,x^{(p)})$ or the sum function $r(\boldsymbol{x})=x^{(1)}+\dots+x^{(p)}$. This allows the creation of two new univariate random variables $R_1=r(\boldsymbol{X}_1)$ and $R_2=r(\boldsymbol{X}_2)$. Points are then considered extreme when the random variable $R_i$ exceeds a given high quantile $q_{u,i}$ corresponding to a high exceedance probability $u\in(0,1)$, $i=1,2$. The set $\{R_i>q_{u,i}\}$ contains the extreme points. This set is then partitioned into a fixed number $W$ of disjoint sets $A_{i,1},\dots,A_{i,W}$. 
Now suppose that we have two random samples $\boldsymbol{x}_{1,1},\dots, \boldsymbol{x}_{1,T}$ and $\boldsymbol{x}_{2,1},\dots,\boldsymbol{x}_{2,T}$. The empirical probability of being in each set $A_{j,w}$ is computed as
\begin{equation}
    \hat{p}_{i,w}=\frac{\sum_{t=1}^T\ind\{\boldsymbol{x}_{i,t}\in A_{i,w}\}}{\sum_{t=1}^T\ind\{r(\boldsymbol{x}_{i,t})>q_{u,i}\}}, \; w=1,\dots W, \; i=1,2, \; t=1, \dots, T.
\end{equation}
Then, the difference in the extremes between the two distributions can be measured with the Kullback–Leibler divergence between two multinomial distributions, defined as
\begin{equation}
    d_{12}=\frac{1}{2}\sum_{w=1}^W\left( \left(  \hat{p}_{1,w}-\hat{p}_{2,w}\right) \log\left(  \hat{p}_{1,w}/\hat{p}_{2,w}\right) \right).
\end{equation}
The choice of the free parameter $W$ presents a classical bias–variance trade-off. A large $W$ allows subtle differences in the extremes to be captured, but if $W$ is too large, the estimation of probabilities becomes highly variable and may lead to the divergence being undefined.

\subsubsection{Dissimilarity measure based on multivariate comonotonicity}
\citet{durante2025clustering} recently proposed a dissimilarity measure based on multivariate comonotonicity. When $p=1$, a copula-based dissimilarity measure can be constructed by quantifying the discrepancy between the copula $C_{XY}$ associated with the random pair $(X,Y)$ and the Fréchet–Hoeffding upper bound $M(u,v)=\min(u,v)$, the comonotonicity copula \citep{fuchs2021dissimilarity}. However, for $p\geq2$, there does not exist a unique notion of comonotonicity. One way to generalize it is through the notion of strong comonotonicity, which states \citep{durante2016principles,puccetti2010multivariate}:
\begin{theorem}\label{thm:strong comonotonicity}
Let $\boldsymbol{X}$ and $\boldsymbol{Y}$ be two random vectors in $\mathrm{L}^0(\mathbb{I}^p)$ with copula $C_{(\boldsymbol{X},\boldsymbol{Y})}.$ Then the following statements are equivalent: 
\begin{enumerate}
    \item $(\boldsymbol{X},\boldsymbol{Y})$ is strongly comonotonic.
    \item The copula $C_{(\boldsymbol{X},\boldsymbol{Y})}=M(\boldsymbol{u},\boldsymbol{v})=\min(u_1,\dots,u_p,v_1,\dots,v_p)$ for all $(\boldsymbol{u},\boldsymbol{v})\in \mathbb{I}^{2p}$.
    \item The copula associated with any pair extracted from $(\boldsymbol{X},\boldsymbol{Y})$ is given by $M$.
\end{enumerate}
\end{theorem}
Here, $\mathrm{L}^0(\mathbb{I}^p)$ denotes the space of all $p$-dimensional random vectors with uniform margins on $\mathbb{I}:=[0,1]$. This notion is extremely strong, as it requires that every element of $\boldsymbol{X}$ is comonotonic with every element of $\boldsymbol{Y}$, and that the elements within $\boldsymbol{X}$ (or $\boldsymbol{Y}$) are also pairwise comonotonic. Another notion of comonotonicity is the $\pi$-comonotonicity, formalized by \citet[Theorem~3.7]{puccetti2010multivariate}, which can be expressed as follows:
\begin{theorem}\label{thm:pi comonotonicity}
Let $\boldsymbol{X}$ and $\boldsymbol{Y}$ be two random vectors in $\mathrm{L}^0(\mathbb{I}^p)$ with copula $C_{(\boldsymbol{X},\boldsymbol{Y})}.$ Then the following statements are equivalent:
\begin{enumerate}
    \item $(\boldsymbol{X},\boldsymbol{Y})$ is $\pi$-comonotonic.
    \item The copula $C_{(\boldsymbol{X},\boldsymbol{Y})}=M(\boldsymbol{u},\boldsymbol{v})=C(M(u_1,v_1),\dots,M(u_p,v_p))$ for all $(\boldsymbol{u},\boldsymbol{v}) \in \mathbb{I}^{2p}$, where $C_{\boldsymbol{X}}=C_{\boldsymbol{Y}}=C$ for a $p$-dimensional copula $C$.
    \item For all $j\in \{1,\dots,p\}$, $C_{(X_j,Y_j)}=M$.
\end{enumerate}
\end{theorem}
Any mapping $d_{\pi}:\mathrm{L}^0(\mathbb{I}^p)\times\mathrm{L}^0(\mathbb{I}^p)\rightarrow[0,+\infty[$ is a dissimilarity function based on $\pi$-comonotonicity if it satisfies $d_{\pi}(\boldsymbol{X},\boldsymbol{Y})=0$ for all $\boldsymbol{X}$ and $\boldsymbol{Y}$ that are $\pi$-comonotonic, and if $d_{\pi}(\boldsymbol{X},\boldsymbol{Y})=d_{\pi}(\boldsymbol{Y},\boldsymbol{X})$. A $(1,1)$-dissimilarity function $d^{1,1}$ is a mapping from $\mathrm{L}^0(\mathbb{I})\times\mathrm{L}^0(\mathbb{I})$ that is law-invariant, symmetric in its arguments, and satisfies $d^{1,1}(X,Y)=0$ when the random pair $(X,Y)$ is coupled by the copula $M$. From Theorem~\ref{thm:pi comonotonicity} (3), we see that we can create a dissimilarity function $d_{\pi}$ by measuring the discrepancy between $C_{(X_j,Y_j)}$ and the copula $M$ for each $j=1,\dots, p$ which can be done easily if we have at our disposal $(1,1)$-dissimilarity function. For example $d_{\pi}^{\max}(\boldsymbol{X},\boldsymbol{Y})
= \max\limits_{j=1,\dots,p} d^{1,1}(X_j, Y_j)$, or $d_{\pi}^{ave}(\boldsymbol{X},\boldsymbol{Y})=1/p\sum\limits_{j=1}^pd^{1,1}(X_j,Y_j)$. Various choices of $d^{1,1}$ can be found in \citet{fuchs2021dissimilarity}.

\subsubsection{Clustering based on Asymptotic Independent Blocks}

\citet{boulin2025high} introduce a model-based clustering framework for multivariate extremes based on \emph{Asymptotic Independent-block (AI-block) models}. Their approach exploits the extremal dependence structure of a weakly dependent multivariate process and defines clusters as subsets of variables whose block maxima remain asymptotically dependent, while different clusters exhibit asymptotic independence.

Consider a $d$-variate stationary and mixing process $(Z_t)_{t\in\mathbb{Z}}$. For a block size $m$, let
$$
M_{m,i}=\left(\max_{t\in((i-1)m,im]} Z_t^{(1)},\dots,\max_{t\in((i-1)m,im]} Z_t^{(d)}\right),
\qquad i=1,\dots,k=\lfloor n/m\rfloor,
$$
denote the componentwise block maxima. Under mild mixing conditions, the copula of $M_{m,1}$ converges to an extreme-value copula $C_\infty$.

\paragraph{AI-block model.}
Let $\mathcal{O}=\{O_1,\dots,O_G\}$ be a partition of $\{1,\dots,d\}$. The process $Z_t$ follows an AI-block model with partition $\mathcal{O}$ if the limiting extreme-value distribution $H$ satisfies
$$
H(x)=\prod_{g=1}^G H^{(O_g)}(x_{O_g}),
$$
i.e., the subvectors $X(O_1),\dots,X(O_G)$ of the limiting extreme-value vector $X$ are mutually independent. This induces a population clustering determined by the extremal dependence structure.

\paragraph{Identifiability.}
Let $\mathcal{L}(Z)$ be the set of partitions for which the AI-block property holds, ordered by refinement. The following result ensures identifiability.

\begin{theorem}[Boulin et al., 2023]
The set $\mathcal{L}(Z)$ admits a unique maximal element $\bar{\mathcal{O}}$, which is the thinnest partition for which the asymptotic independence property holds. This partition represents the population-level clustering of variables under the AI-block model.
\end{theorem}

\paragraph{Extremal coefficients and SECO.}
For an extreme-value vector $X\in\mathbb{R}^d$, the extremal coefficient is defined as
$$
\theta = d\,A(1/d,\dots,1/d),
$$
where $A$ is the Pickands dependence function. For a partition $\mathcal{O}=\{O_g\}_{g=1}^G$, define the \emph{Sum of Extremal Coefficients (SECO)} as
$$
\mathrm{SECO}(\mathcal{O}) = \sum_{g=1}^G \theta(O_g)\;-\;\theta.
$$
Then $\mathrm{SECO}(\mathcal{O})=0$ if and only if $X(O_1),\dots,X(O_G)$ are independent. SECO can thus be used as a diagnostic and as a tuning criterion for data-driven threshold selection.

\paragraph{Pairwise extremal correlation.}
The bivariate extremal coefficient $\theta(a,b)$ satisfies
$$
\theta(a,b)=2-\chi(a,b),
$$
where $\chi(a,b)$ is the extremal correlation. Under an AI-block model,
$$
a\sim_{\bar{\mathcal{O}}} b \quad \Longleftrightarrow\quad \chi(a,b)>0,
\qquad
a\not\sim_{\bar{\mathcal{O}}} b \quad \Longleftrightarrow\quad \chi(a,b)=0,
$$
so the population partition can be recovered via suitable thresholding of pairwise extremal correlations.

\paragraph{Estimation via sub-asymptotic block maxima.}
Given block maxima $M_{m,1},\dots,M_{m,k}$, the extremal coefficient is estimated via a multivariate madogram:
$$
\hat{\nu}_{n,m}=\frac{1}{k}\sum_{i=1}^k
\left(
\max_{j\in\{1,\dots,d\}} U_{m,i}^{(j)} - \frac{1}{d}\sum_{j=1}^d U_{m,i}^{(j)}
\right),
$$
where $U_{m,i}^{(j)}$ are empirical uniform margins. Then
$$
\hat{\theta}_{n,m} = \frac{1/2+\hat{\nu}_{n,m}}{1/2-\hat{\nu}_{n,m}},
\qquad
\hat{\chi}_{n,m}(a,b)=2-\hat{\theta}_{n,m}(a,b).
$$

Under algebraic $\varphi$-mixing, non-asymptotic concentration bounds show that $\hat{\chi}_{n,m}(a,b)$ deviates from its sub-asymptotic target at rate $O(k^{-1/2}+k^{-1})$.

\paragraph{ECO algorithm.}
The authors propose a greedy clustering algorithm called ECO (Extremal COrrelation). Let $\hat{X} = (\hat{\chi}(a,b))$ and let $\tau$ be a threshold.

\begin{algorithm}[H]
\caption{ECO clustering for AI-block models}
\begin{algorithmic}[1]
\State $S\gets\{1,\dots,d\}$, $l\gets 0$
\While{$S\neq\emptyset$}
  \State $l\gets l+1$
  \If{$|S|=1$} \State $\hat{O}_l=S$
  \Else
     \State $(a_l,b_l)=\arg\max_{a,b\in S}\hat{\chi}(a,b)$
     \If{$\hat{\chi}(a_l,b_l)\le\tau$}
        \State $\hat{O}_l=\{a_l\}$
     \Else
        \State $\hat{O}_l=\{s\in S:\hat{\chi}(a_l,s)\wedge \hat{\chi}(b_l,s)\ge\tau\}$
     \EndIf
  \EndIf
  \State $S\gets S\setminus\hat{O}_l$
\EndWhile
\State \Return $\hat{\mathcal{O}}=\{\hat{O}_l\}$
\end{algorithmic}
\end{algorithm}

This procedure does not require prior knowledge of the number of clusters.

\paragraph{Consistency in high dimensions.}
Define the minimal within-cluster extremal correlation
$$
\mathrm{MECO}(X)=\min_{a\sim_{\bar{\mathcal{O}}} b}\chi(a,b)>0.
$$
Under AI-block assumptions, algebraic $\varphi$-mixing, and an appropriate choice of $\tau$ (depending on $d$, $k$, and sub-asymptotic bias $d_m$), the ECO algorithm recovers $\bar{\mathcal{O}}$ with high probability. In particular, if $\mathrm{MECO}(X)$ exceeds an explicit separation bound, then
$$
\mathbb{P}\big( \hat{\mathcal{O}}=\bar{\mathcal{O}} \big)
\ge 1 - 2(1+\sqrt{e})\, d^{-2\gamma}.
$$

\paragraph{Data-driven threshold selection.}
To choose $\tau$ in practice, the authors propose minimizing the empirical SECO criterion
$$
\widehat{\mathrm{SECO}}_{n,m}(\hat{\mathcal{O}})=
\sum_{g} \hat{\theta}( \hat{O}_g ) - \hat{\theta}.
$$
Among a grid of candidate thresholds, one selects the \emph{largest} $\tau$ achieving the minimum, yielding a partition consistent with asymptotic independence while avoiding over-fragmentation.



==> unused_source_files/SwissCatchementApplication.tex <==


\label{sec:camelsch_data}

This application investigates whether Swiss catchments can be grouped according to the complete extremal dependence structure linking liquid precipitation, snowpack depletion, and runoff response. We hypothesize that different flood-generating environments produce distinct angular distributions: primarily rainfall-driven catchments should concentrate toward the liquid-rain--runoff edge of the simplex, snow-dominated Alpine catchments toward the snowmelt--runoff edge, and transitional catchments should exhibit greater interior mass associated with mixed rain--snowmelt--runoff events. Catchment elevation, climatic regime, snow-cover characteristics, and other physical attributes are not used in the clustering; they are examined only afterwards to determine whether the clusters obtained with the Wasserstein--Aitchison method admit a coherent hydrological interpretation.

We used version 0.8 of the Catchment Attributes and Meteorology for Large-sample Studies--Switzerland data set, CAMELS-CH \citep{hoge2023camelsch,hoge2023camelschdata}. CAMELS-CH contains daily hydrometeorological time series and catchment attributes for 331 hydrological units in hydrologic Switzerland, comprising 298 river catchments and 33 lakes. The domain includes catchments within Switzerland and Liechtenstein as well as transboundary catchments in Austria, France, Germany, and Italy. The complete data set covers 1 January 1981--31 December 2020.

We used the observation-based CAMELS-CH time-series collection. For catchment $i$ and day $t$, the variables entering the analysis were catchment-mean precipitation $p_{i,t}$ ($\mathrm{mm}\,\mathrm{d}^{-1}$), catchment-mean daily air temperature $T_{i,t}$ ($^\circ\mathrm{C}$), snow water equivalent $s_{i,t}$ ($\mathrm{mm}$), and observed specific discharge $q_{i,t}$ ($\mathrm{mm}\,\mathrm{d}^{-1}$). Precipitation and temperature originate from the 2-km gridded observation-based products of MeteoSwiss and were spatially averaged over each catchment. Discharge was recorded at the corresponding gauging stations and converted to specific discharge. The discharge observations for 2019--2020 were classified as provisional when CAMELS-CH was released \citep{hoge2023camelsch}.

The snow water equivalent data were provided by the WSL Institute for Snow and Avalanche Research. These data were obtained by aggregating a distributed 1-km snow-cover product constrained by observations from 345 snow-monitoring stations and MeteoSwiss precipitation data; the associated data-assimilation methodology is described by \citet{magnusson2014swe}. Although included in the observation-based part of CAMELS-CH, snow water equivalent is therefore a model--data-assimilation product rather than a direct catchment-scale measurement. Snow water equivalent is available only from September 1998, which determined the analysis period of 1 September 1998--31 December 2020. CAMELS-CH does not provide snow water equivalent for catchments smaller than $10~\mathrm{km}^2$, and estimates in catchments extending above $3000~\mathrm{m}$ a.s.l.\ are subject to increased uncertainty \citep{hoge2023camelsch}.

Daily precipitation was partitioned into liquid and solid fractions using the temperature-dependent liquid fraction
\begin{equation}
f(T)
=
\begin{cases}
0,   & T\leq 0\,^\circ\mathrm{C},\\[2mm]
T/2, & 0\,^\circ\mathrm{C}<T<2\,^\circ\mathrm{C},\\[2mm]
1,   & T\geq 2\,^\circ\mathrm{C}.
\end{cases}
\label{eq:rain_fraction}
\end{equation}
Linear mixing between lower and upper air-temperature thresholds is a common parsimonious representation of mixed-phase precipitation in hydrological and snow models \citep{jennings2019phase}. The limits in equation~\eqref{eq:rain_fraction} place the 50\% liquid fraction at $1\,^\circ\mathrm{C}$, equal to the mean rain--snow threshold obtained by \citet{jennings2018threshold} from 17.8 million Northern Hemisphere observations. That study found that the station-specific 50\% threshold varied from approximately $-0.4$ to $2.4\,^\circ\mathrm{C}$ for 95\% of the stations. Consequently, the interval $0$--$2\,^\circ\mathrm{C}$ should be interpreted as a transparent, spatially uniform phase-partitioning approximation; it does not represent the effects of humidity, atmospheric pressure, or within-catchment elevation variability.

The daily variables were converted into three event-scale coordinates. Liquid precipitation accumulated over the current and two preceding days was defined as
\begin{equation}
L_{i,t}
=
\sum_{j=0}^{2}
p_{i,t-j}f\!\left(T_{i,t-j}\right).
\label{eq:liquid_rain}
\end{equation}
Snowpack water release was represented by the positive net depletion of snow water equivalent over three days,
\begin{equation}
M_{i,t}
=
\left(s_{i,t-3}-s_{i,t}\right)_{+},
\qquad
(x)_{+}=\max(x,0).
\label{eq:swe_depletion}
\end{equation}
Finally, to allow for a short delay between meteorological forcing and the daily discharge response, runoff was represented by the maximum specific discharge on the anchor day or either of the following two days,
\begin{equation}
Q^{\star}_{i,t}
=
\max_{h\in\{0,1,2\}}q_{i,t+h}.
\label{eq:runoff_response}
\end{equation}
Thus, $L_{i,t}$ is a three-day accumulation, $M_{i,t}$ is a three-day net storage change, and $Q^{\star}_{i,t}$ is a three-day response maximum.

The use of a short multi-day window is physically motivated by the event-scale response of Alpine catchments. In an analysis of more than \num{4000} floods from 101 Swiss catchments, \citet{froidevaux2015flood} found that precipitation during the few days immediately preceding a flood was generally the most relevant, and concluded that a three- to four-day precipitation period was sufficient to represent flood triggering in many Swiss Alpine catchments. Moreover, parallel three-day precipitation totals and net three-day snow-water-equivalent decreases have previously been used to distinguish rainfall-driven, snowmelt-driven, and mixed rainfall--snowmelt runoff events \citep{davenport2020flood}. These studies motivate the event timescale of equations~\eqref{eq:liquid_rain}--\eqref{eq:runoff_response}; they do not imply that the precise three-day window or the two-day runoff lead is a universal catchment-response time.

Net snow-water-equivalent depletion is a proxy for snowpack water release rather than a direct estimate of gross snowmelt. Melt occurring concurrently with new snowfall can therefore be partly or completely masked by increasing snow water equivalent. Conversely, a negative snow-water-equivalent change is set to zero rather than being interpreted as negative melt. This definition was chosen because gross snowmelt flux is not available in the observation-based CAMELS-CH time series and because net depletion can be constructed consistently across all eligible catchments. Negative precipitation, snow water equivalent, or discharge values were treated as missing. No missing snow-water-equivalent value was replaced by zero. A derived daily triplet
\[
\bX_{i,t}
=
\left(
L_{i,t},M_{i,t},Q^{\star}_{i,t}
\right)
\]
was retained only when all quantities required by equations~\eqref{eq:liquid_rain}--\eqref{eq:runoff_response} were finite. Catchments with fewer than \num{3650} complete triplets, corresponding approximately to 10 years of daily data, were excluded. This selection was based exclusively on data availability; no catchment was selected using elevation, snow regime, geographical location, angular behavior, or clustering results.

Within each retained catchment, the three margins were transformed separately to standard Pareto scale. Because liquid-rain and snow-water-equivalent-depletion series contain substantial point masses at zero, tied observations were assigned reproducible random ranks within their tie blocks. For a marginal sample of size $n_i$, the transformation was
\[
U_{i,t,j}
=
\frac{\operatorname{rank}(X_{i,t,j})}{n_i+1},
\qquad
Z_{i,t,j}
=
\frac{1}{1-U_{i,t,j}},
\qquad
j=1,2,3.
\]
The $L_1$ radial magnitude was then $r_{i,t}=\sum_{j=1}^{3}Z_{i,t,j}$, and observations above the catchment-specific 95th percentile of $r_{i,t}$ were identified as multivariate extremes. Successive exceedance dates separated by at most three days were assigned to the same event, and only the observation with the largest radial magnitude in each event was retained. The resulting angular observations were transformed to two-dimensional Aitchison coordinates. Empirical angular measures were compared using the $1$-Wasserstein distance and clustered using partitioning around medoids.

\label{sec:camelsch_results}

We fitted partitioning around medoids solutions with $K=2,\ldots,6$ using the pairwise Wasserstein--Aitchison dissimilarities. Appendix~\ref{sec:supplementary_applications} displays the silhouette criterion for values of $K$ ranging from 2 to 6. The maximum was attained for $K=3$, which was therefore retained for the subsequent interpretation.

The resulting partition exhibits broad spatial organization without forming strictly contiguous regions, as shown in Fig.~\ref{fig:camelsch_map}. This is expected because geographical coordinates and spatial adjacency were not used in the clustering. Cluster C1 forms a comparatively small group concentrated mainly among Alpine catchments, whereas C2 and C3 are more widely distributed across the study domain. The spatial pattern therefore indicates that the clusters are related to regional hydroclimatic conditions, while the occurrence of different clusters in neighboring catchments suggests that the partition is not simply reproducing geographical proximity.

\begin{figure}
    \centering
    \includegraphics[width=0.85\textwidth]
    {camels_ch_cluster_point_map_K3.pdf}
    \caption{Spatial distribution of the three extremal-dependence clusters obtained by partitioning around medoids. Red circles, green triangles, and blue squares denote clusters C1, C2, and C3, respectively. Each symbol is placed within the corresponding catchment polygon. The larger symbols surrounded by a black circle identify the medoids: catchments 2269, 2210, and 2181 for C1, C2, and C3, respectively. Light-grey lines delimit the catchments included in the clustering. Spatial position and catchment geometry were not used to construct the clusters, and the labels C1--C3 have no ordinal meaning.}
    \label{fig:camelsch_map}
\end{figure}

Figure~\ref{fig:camelsch_simplex} displays the empirical angular measures of the three medoids. The medoid of C1 has the most broadly dispersed angular measure. In addition to substantial mass near the rain vertex and along the liquid-rain--runoff edge, it contains comparatively more observations in melt-related directions, including along the snowmelt--runoff edge and in the simplex interior. Consistently, this medoid has the largest of the three rain--melt and melt--runoff tail-dependence estimates, $\widehat\chi(L,M)=0.16$ and $\widehat\chi(M,Q^\star)=0.25$, while its rain--runoff coefficient is $\widehat\chi(L,Q^\star)=0.33$.

The C2 medoid exhibits an intermediate configuration. Its angular mass is distributed between rain-dominated observations, melt-dominated observations, and events lying along the liquid-rain--runoff and snowmelt--runoff edges. Its pairwise coefficients,
\[
\widehat\chi(L,M)=0.13,\qquad
\widehat\chi(L,Q^\star)=0.38,\qquad
\widehat\chi(M,Q^\star)=0.21,
\]
are intermediate between those of C1 and C3. This group is consequently interpreted as a transitional regime rather than as a purely rainfall- or snowmelt-controlled regime.

In contrast, the angular measure of the C3 medoid is strongly concentrated near the liquid-rain--runoff edge. Its rain--runoff coefficient, $\widehat\chi(L,Q^\star)=0.60$, is substantially larger than its rain--melt and melt--runoff coefficients, which are respectively $0.09$ and $0.13$. C3 therefore represents the clearest rainfall--runoff extremal dependence regime.

The simplex distributions also qualify the hypothesis formulated before the analysis. The anticipated contrast between a snow-influenced regime and a rainfall--runoff regime is visible. However, none of the three medoids exhibits a dominant concentration near the centre of the simplex. Most angular observations remain close to a vertex or an edge. Thus, the results do not support the existence of a large class characterized primarily by balanced three-variable extremes. Instead, C2 represents a heterogeneous transition between rain- and melt-related extremal configurations.

\begin{figure}
    \centering
    \includegraphics[width=\textwidth]
    {camels_ch_medoid_simplex_with_chi_K3.pdf}
    \caption{Empirical angular measures of the medoids for $K=3$. From left to right, the panels correspond to C1, catchment 2269, C2, catchment 2210, and C3, catchment 2181. Each point represents one runs-declustered multivariate extreme event retained at the corresponding medoid catchment. The vertices represent dominance of standardized liquid rainfall, $L$, net snow-water-equivalent depletion, $M$, and runoff response, $Q^\star$. Points along an edge indicate that the two corresponding standardized variables dominate the third, whereas interior points indicate appreciable contributions from all three variables. The coordinates are proportions of the standard-Pareto-transformed variables and must not be interpreted as physical water-budget fractions. The displayed pairwise tail-dependence summaries are $\widehat\chi_{ab}=3n^{-1}\sum_{r=1}^{n}\min(\Theta_{r,a},\Theta_{r,b})$ and are calculated only for the displayed medoid. The number above each panel is the number of declustered events contributing to its empirical angular measure.}
    \label{fig:camelsch_simplex}
\end{figure}

The pairwise coefficients provide useful summaries of the dominant relationships, particularly the strong liquid-rain--runoff association in C3. They do not, however, describe how angular mass is divided among the vertices, different parts of the edges, and asymmetric interior regions. For example, the complete angular measures reveal the broader dispersion of C1 and the mixture of distinct rain- and melt-related configurations in C2. These distributional features are precisely the information incorporated by the Wasserstein--Aitchison dissimilarity.

The hydrological interpretation was evaluated using four CAMELS-CH attributes that were excluded from the clustering: mean catchment elevation, the fraction of precipitation falling as snow, mean catchment slope, and mean half-flow date, as shown in Fig.~\ref{fig:camelsch_validation}. The half-flow date is the number of days from the beginning of the hydrological year, defined as 1 October, required for cumulative discharge to reach one half of annual discharge \citep{hoge2023camelsch}.

C1 catchments have the highest mean elevations and the largest fractions of precipitation falling as snow. They also have steeper slopes and later half-flow dates, consistent with delayed runoff associated with seasonal snow storage and melt. C3 catchments have the lowest elevations and snow fractions, supporting their interpretation as predominantly rainfall--runoff catchments. C2 occupies an intermediate position for elevation and snow fraction, consistent with its transitional angular distribution.

The three clusters are pairwise distinguishable in terms of both mean catchment elevation and snow fraction. For mean slope and half-flow date, C1 differs from C2 and C3, whereas C2 and C3 are not distinguishable after multiple-testing correction. Elevation and snow fraction are themselves closely related in Alpine environments, so they should not be regarded as independent validation signals. Nevertheless, their agreement with the angular geometry, together with the differences in slope and half-flow timing, provides external support for the hydrological interpretation of the clusters.

% \begin{figure}
%     \centering
%     \includegraphics[width=\textwidth]
%     {camels_ch_final_attribute_validation.pdf}
%     \caption{External physical validation of the three extremal-dependence clusters. The panels show box plots of mean catchment elevation, fraction of precipitation falling as snow, mean catchment slope, and mean half-flow date, measured in days since 1 October. Individual symbols represent catchments: circles, triangles, and squares correspond to C1, C2, and C3, respectively. Lowercase letters are significance-group labels. Clusters sharing a letter are not significantly different, whereas clusters with no letter in common differ at the 5\% level according to pairwise Wilcoxon rank-sum tests. None of these validation attributes was used in the Wasserstein--Aitchison clustering.}
%     \label{fig:camelsch_validation}
% \end{figure}

==> unused_source_files/notes.tex <==


\subsection{Notation}
Let \(n \geq 2\) denote the number of grid cells at which we have \(p \geq 2\) dimensional time series at time step $t$. For grid cell $i \in \{1,\dots,n\}$, and time step $t$ we have the following $p$-dimensional random vector
\[
\bX_{i,t} = \left(X_{i,t}^{(1)},\dots,X_{i,t}^{(p)}\right).
\]
We assume that observations are available over $T$ time steps. For each $t \in \{1,\dots,T\}$, let
$$
\bx_{i,t} = \left(x_{i,t}^{(1)},\dots,x_{i,t}^{(p)}\right) \in \mathbb{R}^p
$$
denote the realization of $\bX_{i,t}$ at time $t$. The corresponding sample associated with grid cell $i$ is therefore given by $\left(\bx_{i,t}\right)_{t=1,\dots,T}$. The collection of all random vectors is denoted by $\mathcal{X} = \left\{\bX_1,\dots,\bX_n\right\}$. The objective is to construct a partition of $\mathcal{X}$ by exploiting the dependence structure between its elements. Most clustering methodologies considered in this work follow three main steps:
\begin{enumerate}
    \item Define a dissimilarity measure between the elements of $\mathcal{X}$,
    \item Construct the associated dissimilarity matrix $ \bD \in \mathbb{R}^{n \times n}$,
    \item Apply a clustering algorithm, such as hierarchical clustering or \(k\)-medoids, to the resulting matrix.
\end{enumerate}

\subsection{Compound Clustering: State of the art}

Because our work focuses on spatial time series data. We first present the methodology of \citet{benevento2025comonotonic}, which consists of clustering spatial univariate time series based on comonotonicity. Since raw observations may exhibit trends, seasonality, serial dependence, or heteroscedasticity, each marginal time series is first filtered. Let $(\hat{\epsilon}_{i,t})_{t=1,\dots,T}$ denote the residual series obtained after marginal filtering. The filtering step is chosen such that the residuals behave approximately as independent and identically distributed observations for each fixed grid cell $i$. Their idea is to focus on the copula of the residuals. Hence, to remove the influence of the marginal distributions, they transform the residuals into pseudo-observations through the empirical distribution functions. For each $i$ and each $t$, define $\hat{U}{i,t}=\hat{F}_i(\hat\epsilon_{i,t})$, where $\hat{F}_i$ is the empirical distribution function of the residual series at grid cell $i$.For each pair of grid cells $(i,j)$, the dependence structure between the transformed series
$(\hat{U}_{t,i},\hat{U}_{t,j})_{t=1,\dots,T}$ is described by the associated empirical copula
\begin{equation}
    \hat{C}_{ij}(u,v)
=
\frac{1}{T}
\sum_{t=1}^T
\ind\left\{
\hat{U}_{t,i}\leq u,\,
\hat{U}_{t,j}\leq v
\right\},
\qquad
(u,v)\in[0,1]^2.
\label{eq:bivariate_empirical_copula}
\end{equation}
They then propose to compare the empirical copula $\hat{C}_{ij}(u,v)$ to the comonotonicity copula $M(u,v)=\min(u,v)$, which corresponds to perfect positive dependence. A dissimilarity measure is therefore defined through a distance between $\hat{C}_{ij}(u,v)$ and $M$:
$$
\Delta^{ts}_{ij}
=
d^{1,1}(\hat{C}_{ij},M),
$$
where $d^{1,1}$ denotes a suitable metric on the space of bivariate copulas. The pairwise dissimilarities are then assembled into the matrix
\begin{equation}
    \bD^{ts}
=
(\Delta_{ij})_{i,j=1,\dots,n}
\in \mathbb{R}^{n\times n},
\label{eq:dissimilarity_matrix}
\end{equation}
The superscript $ts$ refers to the fact that this dissimilarity captures the temporal synchronicity between the different stations.

To capture the spatial dependence, they propose to construct a second dissimilarity matrix $\bD^{sp}$, where the dissimilarity is now based on geographic information. More precisely, let $\svec_i$ denote the geographic coordinates corresponding to the latitude and longitude of the center of grid cell $i$. They then propose to construct $\bD^{sp}_{ij}$ either as a binary matrix encoding neighbouring cells, or as a distance matrix based on a kernel that decays with the distance, namely $K(\|\svec_i-\svec_j\|)$. Note that these feature vectors are deterministic and fixed across time. By constructing this matrix, their goal is to enforce spatial coherence during the clustering procedure.

Finally, they propose to construct a global dissimilarity matrix $\bD^{\alpha}$, with $\alpha\in[0,1]$, which consists of a mixture of the two matrices. The matrix $\bD^{\alpha}$ is finally used as input for a clustering algorithm such as hierarchical clustering or \(K\)-medoids. The overall methodology can therefore be summarized by the following pipeline:
$$
\begin{array}{cccc}
(X_{t,i})
\longrightarrow
(\hat{\epsilon}_{t,i})
\longrightarrow
(\hat{U}_{t,i})
\longrightarrow
\hat{C}_{ij}
\longrightarrow
\Delta^{ts}_{ij}
\\[1em]
(\svec_i,\svec_j)
\longrightarrow
\Delta^{sp}_{ij}
\end{array}
\qquad
\left.
\begin{array}{c}
\\[-0.6em]
\\[-0.2em]
\end{array}
\right\}
\longrightarrow
\Delta^{\alpha}_{ij}
\longrightarrow
\bD^{\alpha}
\longrightarrow
\text{clustering}.
$$

\citet{vignotto2021clustering} proposed a clustering methodology for compound extremes based on a dissimilarity measure derived from the Kullback--Leibler (KL) divergence. The objective is to compare the extremal dependence structures of multivariate distributions across different spatial locations. In the present framework, we assume that the marginal filtering step described previously has already been performed. Consequently, for each grid cell $i$, we directly consider the filtered residual vectors
$$
\hat{\boldsymbol{\epsilon}}_{i,t}
=
\left(
\hat\epsilon_{i,t}^{(1)},
\dots,
\hat\epsilon_{i,t}^{(p)}
\right),
\qquad
t=1,\dots,T.
$$
The methodology first transforms each marginal distribution to the standard Pareto scale. For each component $k=1,\dots,p$, let $\hat{F}_{i,k}$ denote the empirical distribution function associated with the residual series $(\hat\epsilon_{i,t}^{(k)})_{t=1,\dots,T}$. The transformation is then defined by
\begin{equation}
    Z_{i,t}^{(k)}
    =
    \frac{1}{
    1-\hat{F}_{i,k}(\hat\epsilon_{i,t}^{(k)})
    }.
    \label{eq:transform_pareto}
\end{equation}
This transformation places all margins on a common scale. To identify extreme regions, they introduce a risk function $ r : \Rset \to \Rset$,
applied to the Pareto-transformed observations. Typical choices include
$$
r(\boldsymbol{z})=\max\left(z^{(1)},\dots,z^{(p)}\right)
\quad \text{or} \quad
r(\boldsymbol{z})=z^{(1)}+\dots+z^{(p)}.
$$
For each grid cell $i$, they define $ \boldsymbol{Z_{i,t}} = \left(Z_{i,t}^{(1)},\dots,Z_{i,t}^{(p)}\right)$ and the associated univariate random variables $ R_{i,t} = r(\boldsymbol{Z}_{i,t})$.

A point is considered extreme whenever $R_{i,t} > q_{u,i}$, 
where $q_{u,i}$ denotes a high quantile associated with an exceedance probability $u\in(0,1)$. The corresponding tail region is therefore $
\left\{ R_{i,t} > q_{u,i} \right\}$. They proposed to partitioned the extreme region into $W$ disjoint subsets $A_{i,1},\dots,A_{i,W}$. An illustration of the partitioning procedure for a two dimensional vector is shown in Figure~\ref{fig:vignotto_partition}.

The empirical proportion of extreme observations falling into region $A_{i,w}$ is estimated by
$$
\hat{p}_{i,w}
=
\frac{
\sum_{t=1}^T
\ind\left\{
\boldsymbol{Z}_{i,t}\in A_{i,w}
\right\}
}{
\sum_{t=1}^T
\ind\left\{
R_{i,t}>q_{u,i}
\right\}
},
\qquad
w=1,\dots,W.
$$
The vector $(\hat{p}_{i,1},\dots,\hat{p}_{i,W})$
can therefore be interpreted as empirical multinomial distributions describing how extremes are distributed across the tail regions.

The dissimilarity between the extremal dependence structures of two grid cells $i$ and $j$ is then quantified using the symmetrized KL-divergence
$$
\Delta_{ij}
=
\frac{1}{2}
\sum_{w=1}^W
\left(
\hat{p}_{i,w}-\hat{p}_{j,w}
\right)
\log
\left(
\frac{\hat{p}_{i,w}}{\hat{p}_{j,w}}
\right).
$$
A small value of $\Delta_{ij}$ indicates that both grid cells exhibit similar extremal dependence structures, whereas large values indicate different tail behaviours. Finally, the pairwise divergences are assembled into a dissimilarity matrix $\bD= (\Delta_{ij})_{i,j=1,\dots,n} \in \Rset^{n\times n}$, which is then used as input for a clustering algorithm.

The parameter $W$ controls the resolution of the tail partition. Large values of $W$ allow finer differences in the extremal dependence structure to be detected, but may lead to unstable probability estimates when too few observations fall into each subset. The choice of $W$ therefore induces a classical bias-variance trade-off. It is important to remark that this procedure allow to find region where the tail behavior is similar and not when an extreme event occurs simultaneously in time. 
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\linewidth]{notes_figures/ClusteringVignotto.png}
    \caption{Illustration of the partitioning of the extremal region used in \citet{vignotto2021clustering}. After marginal standardization to the Pareto scale, the tail region is divided into \(W\) disjoint subsets. The empirical proportions of exceedances in these regions are then used to construct the KL-based dissimilarity measure between extremal dependence structures.}
    \label{fig:vignotto_partition}
\end{figure}

While the methodology of \citet{benevento2025comonotonic} focuses on univariate time series, \citet{durante2025clustering} recently proposed an extension to multivariate random vectors based on the notion of multivariate comonotonicity. As in the previous approaches, we assume that the marginal filtering step has already been performed. Consequently, for each grid cell $i$, we directly consider the filtered residual vectors
$$
\hat{\boldsymbol{\epsilon}}_{i,t}
=
\left(
\hat\epsilon_{i,t}^{(1)},
\dots,
\hat\epsilon_{i,t}^{(p)}
\right),
\qquad
t=1,\dots,T,
$$
which are transformed into pseudo-observations using the empirical marginal distribution functions.

When $p=1$, copula-based dissimilarity measures quantify the discrepancy between the copula associated with a pair $(X,Y)$ and the Fréchet--Hoeffding upper bound
$$
M(u,v)=\min(u,v),
\qquad
(u,v)\in[0,1]^2,
$$
which corresponds to perfect positive dependence \citep{fuchs2021dissimilarity}. However, for multivariate random vectors with $p\geq2$, several notions of comonotonicity can be considered.

One possible extension is the notion of strong comonotonicity \citep{durante2016principles,puccetti2010multivariate}. In this framework, two random vectors $\boldsymbol{X}$ and $\boldsymbol{Y}$ are strongly comonotonic when every pair of components extracted from $(\boldsymbol{X},\boldsymbol{Y})$ is comonotonic. Equivalently, the associated copula is given by
$$
M(\boldsymbol{u},\boldsymbol{v})
=
\min(u_1,\dots,u_p,v_1,\dots,v_p),
\qquad
(\boldsymbol{u},\boldsymbol{v})\in[0,1]^{2p}.
$$
This notion is very restrictive since it also imposes comonotonicity between the components within each vector.

To obtain a weaker notion, \citet{puccetti2010multivariate} introduced the concept of $\pi$-comonotonicity. In that case, two random vectors $\boldsymbol{X}$ and $\boldsymbol{Y}$ are said to be $\pi$-comonotonic whenever, for each component $k=1,\dots,p$, the pair $(X_k,Y_k)$ is comonotonic. The corresponding copula can then be written as
$$
M(\boldsymbol{u},\boldsymbol{v})
=
C\left(
M(u_1,v_1),
\dots,
M(u_p,v_p)
\right),
$$
where $C$ denotes the common copula associated with $\boldsymbol{X}$ and $\boldsymbol{Y}$.

Based on this characterization, \citet{durante2025clustering} proposed to construct multivariate dissimilarity measures from bivariate copula-based dissimilarities. Let
$$
d^{1,1}:
\mathrm{L}^0([0,1])
\times
\mathrm{L}^0([0,1])
\rightarrow
[0,+\infty[
$$
denote a bivariate dissimilarity measure satisfying
$$
d^{1,1}(X,Y)=0
$$
whenever the copula associated with $(X,Y)$ is equal to $M$. Various examples of such measures are discussed in \citet{fuchs2021dissimilarity}.

The multivariate dissimilarity between two random vectors $\boldsymbol{X}$ and $\boldsymbol{Y}$ can then be obtained by aggregating the componentwise dissimilarities. For example, they proposed the maximum-based dissimilarity
$$
d_{\pi}^{\max}
(\boldsymbol{X},\boldsymbol{Y})
=
\max_{k=1,\dots,p}
d^{1,1}(X_k,Y_k),
$$
or alternatively the average dissimilarity
$$
d_{\pi}^{ave}
(\boldsymbol{X},\boldsymbol{Y})
=
\frac{1}{p}
\sum_{k=1}^p
d^{1,1}(X_k,Y_k).
$$

In the spatial framework considered in this work, the dissimilarity between two grid cells $i$ and $j$ is therefore obtained by comparing the transformed multivariate series associated with both locations. The pairwise dissimilarities are finally assembled into a matrix
$$
\bD
=
(\Delta_{ij})_{i,j=1,\dots,n}
\in
\mathbb{R}^{n\times n},
$$
which is then used as input for a clustering algorithm such as hierarchical clustering or \(K\)-medoids.


% \subsubsection{Vignotto et al. (2021): KL divergence for extremal dependence clustering}

% \citet{vignotto2021clustering} proposed a clustering methodology for compound extremes based on a dissimilarity measure derived from the Kullback--Leibler (KL) divergence. The objective is to compare the extremal dependence structures of multivariate distributions across different spatial locations. Consider two \(p\)-dimensional random vectors \(\bX_1\) and \(\bX_2\). The methodology first transforms each marginal distribution to the standard Pareto scale. For a univariate random variable \(X\) with cumulative distribution function \(F\), the transformation is given empirically by
% \[
% X \mapsto \frac{1}{1-\hat{F}(X)}.
% \]
% This transformation places all margins on a common scale.

% To identify extreme regions, the authors introduce a risk function
% \[
% r : \mathbb{R}^p \to \mathbb{R},
% \]
% applied to the Pareto-transformed observations. Typical choices include
% \[
% r(\bx)=\max\left(x^{(1)},\dots,x^{(p)}\right)
% \quad \text{or} \quad
% r(\bx)=x^{(1)}+\dots+x^{(p)},
% \]
% and, for \(i=1,2\), define the associated univariate random variables $R_i = r(\bX_i).$
% A point is considered extreme whenever $R_i > q_{u,i},$
% where \(q_{u,i}\) denotes a high quantile associated with an exceedance probability \(u\in(0,1)\). The corresponding tail region is therefore
% \[
% \left\{R_i > q_{u,i}\right\}.
% \]
% The extreme region is then partitioned into \(W\) disjoint subsets
% \[
% A_{i,1},\dots,A_{i,W}.
% \]
% An illustration of the partitioning procedure used in the construction of the KL divergence is shown in Figure~\ref{fig:vignotto_partition}.
% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.75\linewidth]{notes_figures/ClusteringVignotto.png}
%     \caption{Illustration of the partitioning of the extremal region used in \citet{vignotto2021clustering}. After marginal standardization to the Pareto scale, the tail region is divided into \(W\) disjoint subsets. The empirical proportions of exceedances in these regions are then used to construct the KL-based dissimilarity measure between extremal dependence structures.}
%     \label{fig:vignotto_partition}
% \end{figure}
% Suppose now that, for each \(i=1,2\), observations
% \[
% (\bx_{i,t})_{t=1,\dots,T}
% \]
% are available. The empirical proportion of extreme observations falling into region \(A_{i,w}\) is estimated by
% \[
% \hat{p}_{i,w}
% =
% \frac{
% \sum_{t=1}^T
% \ind\left\{
% \bx_{i,t}\in A_{i,w}
% \right\}
% }{
% \sum_{t=1}^T
% \ind\left\{
% r(\bx_{i,t})>q_{u,i}
% \right\}
% },
% \qquad
% w=1,\dots,W.
% \]
% The vectors
% \[
% (\hat{p}_{i,1},\dots,\hat{p}_{i,W})
% \]
% can therefore be interpreted as empirical multinomial distributions describing how extremes are distributed across the tail regions.
% The dissimilarity between the extremal dependence structures of \(\bX_1\) and \(\bX_2\) is then quantified using the symmetrized Kullback--Leibler divergence
% \[
% d_{12}
% =
% \frac{1}{2}
% \sum_{w=1}^W
% \left(
% \hat{p}_{1,w}-\hat{p}_{2,w}
% \right)
% \log
% \left(
% \frac{\hat{p}_{1,w}}{\hat{p}_{2,w}}
% \right).
% \]

% A small value of \(d_{12}\) indicates that both random vectors exhibit similar extremal dependence structures, whereas large values indicate different tail behaviours.
% Finally, the pairwise divergences are assembled into a dissimilarity matrix
% \[
% \bD \in \mathbb{R}^{n\times n},
% \]
% which is then used as input for a clustering algorithm such as \(k\)-medoids.

% The parameter \(W\) controls the resolution of the tail partition. Large values of \(W\) allow finer differences in the extremal dependence structure to be detected, but may lead to unstable probability estimates when too few observations fall into each subset. The choice of \(W\) therefore induces a classical bias--variance trade-off.
% \begin{itemize}

%     \item \textcolor{blue}{\textbf{Temporal dependence.} The methodology of \citet{vignotto2021clustering} is developed for independent observations. However, in climate applications, the observations are typically time series exhibiting strong temporal dependence. As a consequence, the empirical proportions used in the KL divergence may be biased by temporal clustering effects. One possible approach consists in first filtering the temporal dependence structure, for instance through autoregressive modeling or declustering techniques, and then applying the methodology to the residual process.}

%     \item \textcolor{blue}{\textbf{Choice of the partition parameter \(W\).} The construction of the divergence relies on a partition of the tail region into \(W\) disjoint subsets. The choice of \(W\) is somewhat ad-hoc and introduces a bias--variance trade-off: large values of \(W\) allow finer differences in extremal dependence to be detected, but may lead to unstable estimates due to data sparsity in the tail.}

%     \item \textcolor{blue}{\textbf{Possible improvement via angular measures.} A more natural alternative would consist in directly comparing the extremal dependence structures through the empirical angular measure associated with each station. In the bivariate case (\(p=2\)), after standard Pareto normalization, pseudo-polar coordinates can be introduced through
%     \[
%     R = X^{(1)} + X^{(2)},
%     \qquad
%     W = \frac{X^{(1)}}{X^{(1)}+X^{(2)}}.
%     \]
%     Under multivariate regular variation, the conditional distribution
%     \[
%     \mathbb{P}(W \in \cdot \mid R > r)
%     \]
%     converges, as \(r\to\infty\), to the angular measure \(H\) on \([0,1]\). The angular measure characterizes the extremal dependence structure:
%     \begin{itemize}
%         \item concentration around \(1/2\) indicates strong co-extremes,
%         \item concentration near \(0\) and \(1\) indicates asymptotic independence.
%     \end{itemize}
%     One could therefore estimate empirically the angular measure at each station and compare stations directly through a distance between angular measures.}

%     \item \textcolor{blue}{\textbf{Wasserstein distance between angular measures.} Let \(H_i\) and \(H_j\) denote the empirical angular measures associated with stations \(i\) and \(j\). A natural dissimilarity measure is the Wasserstein distance
%     \[
%     \mathcal{W}(H_i,H_j)
%     =
%     \inf_{\pi \in \Pi(H_i,H_j)}
%     \int_{[0,1]^2}
%     |x-y|
%     \, d\pi(x,y),
%     \]
%     where \(\Pi(H_i,H_j)\) denotes the set of couplings having marginals \(H_i\) and \(H_j\). This approach avoids the arbitrary partition parameter \(W\) and provides a geometrically meaningful comparison between extremal dependence structures.}

%     \item \textcolor{blue}{\textbf{Lack of temporal synchronization information.} The proposed divergence measures similarity between tail dependence structures but does not quantify whether extreme events occur simultaneously in time across different locations. Two stations may exhibit very similar extremal dependence structures while their extreme events occur at completely different periods. For compound climate events, temporal synchronization is often crucial and should ideally be incorporated into the clustering methodology.}

% \end{itemize}

% \subsubsection{Comonotonicity-based clustering of time series \citep{benevento2025comonotonic}}
% Consider \(n\) univariate time series observed over \(T\) time steps. For each location \(i\in\{1,\dots,n\}\), let
% \[
% (X_{t,i})_{t=1,\dots,T}
% \]
% denote the observed time series. The objective is to cluster the different locations according to the dependence structure between their time series. More precisely, the methodology focuses on the co-movements between the series, that is, whether large or small values tend to occur simultaneously across locations.

% Since the raw observations may exhibit trends, seasonality, serial dependence, or heteroscedasticity, each marginal series is first filtered individually. Let
% \[
% (\varepsilon_{t,i})_{t=1,\dots,T}
% \]
% denote the residual series obtained after marginal filtering. The filtering step is chosen so that the residuals behave approximately as independent and identically distributed observations for each fixed location \(i\).

% To remove the influence of the marginal distributions, the residuals are transformed into pseudo-observations through their empirical distribution functions. For each \(t=1,\dots,T\) and \(i=1,\dots,n\), define
% \[
% U_{t,i}
% =
% \hat{F}_i(\varepsilon_{t,i}),
% \]
% where \(\hat{F}_i\) denotes the empirical distribution function of the residual series at location \(i\). Equivalently,
% \[
% U_{t,i}
% =
% \frac{\operatorname{rank}(\varepsilon_{t,i})}{T+1}.
% \]

% After this transformation, each marginal distribution is approximately uniform on \([0,1]\), so that the remaining information is entirely contained in the dependence structure between the series.

% For each pair of locations \((i,j)\), the dependence structure between the transformed series
% \[
% (U_{t,i},U_{t,j})_{t=1,\dots,T}
% \]
% is described by the associated empirical copula
% \[
% \hat{C}_{ij}(u,v)
% =
% \frac{1}{T}
% \sum_{t=1}^T
% \ind\left\{
% U_{t,i}\leq u,\,
% U_{t,j}\leq v
% \right\},
% \qquad
% (u,v)\in[0,1]^2.
% \]

% The methodology then compares each empirical copula \(\hat{C}_{ij}\) to the comonotonicity copula
% \[
% M(u,v)=\min(u,v),
% \]
% which corresponds to perfect positive dependence. Intuitively, if \(\hat{C}_{ij}\) is close to \(M\), then extreme or moderate events tend to occur simultaneously in both series.

% A dissimilarity measure is therefore defined through a distance between \(\hat{C}_{ij}\) and \(M\):
% \[
% \Delta_{ij}
% =
% d(\hat{C}_{ij},M),
% \]
% where \(d\) denotes a suitable metric on the space of bivariate copulas.

% The pairwise dissimilarities are then assembled into the matrix
% \[
% \bD
% =
% (\Delta_{ij})_{i,j=1,\dots,n}
% \in \mathbb{R}^{n\times n},
% \]
% which is finally used as input for a clustering algorithm such as hierarchical clustering or \(K\)-medoids.

% The overall methodology can therefore be summarized by the following pipeline:
% \[
% (X_{t,i})
% \quad\longrightarrow\quad
% (\varepsilon_{t,i})
% \quad\longrightarrow\quad
% (U_{t,i})
% \quad\longrightarrow\quad
% \hat{C}_{ij}
% \quad\longrightarrow\quad
% \Delta_{ij}
% \quad\longrightarrow\quad
% \bD
% \quad\longrightarrow\quad
% \text{clustering}.
% \]

